Adversarial Attacks on Time Series

Time series classification models have been garnering significant importance in the research community. However, not much research has been done on generating adversarial samples for these models. These adversarial samples can become a security concern. In this paper, we propose utilizing an adversarial transformation network (ATN) on a distilled model to attack various time series classification models. The proposed attack on the classification model utilizes a distilled model as a surrogate that mimics the behavior of the attacked classical time series classification models. Our proposed methodology is applied onto 1-Nearest Neighbor Dynamic Time Warping (1-NN ) DTW, a Fully Connected Network and a Fully Convolutional Network (FCN), all of which are trained on 42 University of California Riverside (UCR) datasets. In this paper, we show both models were susceptible to attacks on all 42 datasets. To the best of our knowledge, such an attack on time series classification models has never been done before. Finally, we recommend future researchers that develop time series classification models to incorporating adversarial data samples into their training data sets to improve resilience on adversarial samples and to consider model robustness as an evaluative metric.

==> dataset_summary.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
%\newcolumntype{C}{>{\centering\arraybackslash}X}
%\newcommand\mcxl[1]{\multicolumn{1}{|C|}{\bfseries #1}}
%\newcommand\mcx[1]{\multicolumn{1}{C }{\bfseries #1}}
 
\def\tabularxcolumn#1{m{#1}}
\setlength\arrayrulewidth{1pt}


\newcolumntype{b}{>{\centering \arraybackslash\hsize=1.5 \hsize}X}
\newcolumntype{s}{>{\centering \arraybackslash \hsize=.5 \hsize}X}
\newcommand{\heading}[1]{\multicolumn{1}{c}{#1}}

\begin{table*}[]
\centering
\caption{Properties of all datasets. The yellow cells are datasets used by \textit{Pei et al.} \cite{pei2017multivariate}, the purple cells are datasets used by \textit{Sch\"{a}fer and Leser} \cite{schafer2017multivariate}, and the blue cells are datasets from the UCI repository \cite{Lichman:2013}.}
\label{tab:sum_data}
\begin{adjustbox}{width=1 \textwidth}

\begin{tabularx}{1.1 \textwidth}{|b|s|s|s|b|b|c|}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

    \hline
    \textbf{Dataset} & \textbf{Num. of Classes} & \textbf{Num. of Variables} & \textbf{Max Training Length} & \textbf{Task} & \textbf{Train-Test Split} & \textbf{Source}\\
    \hline
    \rowcolor[rgb]{ 1,  .98,  .81} \textbf{OHC} & 20    & 30    & 173   & Handwriting Classification & 10-fold & \cite{williams2008modelling}\\
    \hline
    \rowcolor[rgb]{ 1,  .98,  .81} \textbf{Arabic Voice} & 88    & 39    & 91    & Speaker Recognition & 75-25 split & \cite{hammami2010improved} \\
    \hline
    \rowcolor[rgb]{ 1,  .98,  .81} \textbf{Cohn-Kanade AU-coded Expression (CK+)} & 7     & 136   & 71    & Facial Expression Classification & 10-fold & \cite{van2012action} \\
    \hline
    \rowcolor[rgb]{ 1,  .98,  .81} \textbf{MSR Action} & 20    & 570   & 100   & Action Recognition & 5 ppl in train; rest in test & \cite{li2010action} \\
    \hline
    \rowcolor[rgb]{ 1,  .98,  .81} \textbf{MSR Activity} & 16    & 570   & 337   & Activity Recognition & 5 ppl in train; rest in test & \cite{wang2012mining} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{ArabicDigits} & 10    & 13    & 93    & Digit Recognition & 75-25 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{AUSLAN} & 95    & 22    & 96    & Sign Language Recognition & 44-56 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{CharacterTrajectories} & 20    & 3     & 205   & Handwriting Classification & 10-90 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{CMU\_MOCAP\_S16} & 2     & 62    & 534   & Action Recognition & 50-50 split & \cite{cmu} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{DigitShape} & 4     & 2     & 97    & Action Recognition & 60-40 split & \cite{subakan2014probabilistic} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{ECG} & 2     & 2     & 147   & ECG Classification & 50-50 split & \cite{bobski_world} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{JapaneseVowels} & 9     & 12    & 26    & Speech Recognition & 42-58 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{KickvsPunch} & 2     & 62    & 761   & Action Recognition & 62-38 split & \cite{cmu} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{LIBRAS} & 15    & 2     & 45    & Sign Language Recognition & 38-62 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{LP1} & 4     & 6     & 15    & Robot Failure Recogntion & 43-57 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{LP2} & 5     & 6     & 15    & Robot Failure Recogntion & 36-64 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{LP3} & 4     & 6     & 15    & Robot Failure Recogntion & 36-64 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{LP4} & 3     & 6     & 15    & Robot Failure Recogntion & 36-64 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{LP5} & 5     & 6     & 15    & Robot Failure Recogntion & 39-61 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{NetFlow} & 2     & 4     & 994   & Action Recognition & 60-40 split & \cite{subakan2014probabilistic} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{PenDigits} & 10    & 2     & 8     & Digit Recognition & 2-98 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{Shapes} & 3     & 2     & 97    & Action Recognition & 60-40 split & \cite{subakan2014probabilistic} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{Uwave} & 8     & 3     & 315   & Gesture Recognition & 20-80 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{Wafer} & 2     & 6     & 198   & Manufacturing Classification & 25-75 split & \cite{bobski_world} \\
    \hline
    \rowcolor[rgb]{ .87,  .81,  1} \textbf{WalkVsRun} & 2     & 62    & 1918  & Action Recognition & 64-36 split & \cite{cmu} \\
    \hline
    \rowcolor[rgb]{ .81,  .87,  1} \textbf{AREM} & 7     & 7     & 480   & Activity Recognition & 50-50 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .81,  .87,  1} \textbf{HAR} & 6     & 9     & 128   & Activity Recognition & 71-29 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .81,  .87,  1} \textbf{Daily Sport} & 19    & 45    & 125   & Activity Recognition & 50-50 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .81,  .87,  1} \textbf{Gesture Phase} & 5     & 18    & 214   & Gesture Recognition & 50-50 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .81,  .87,  1} \textbf{EEG} & 2     & 13    & 117   & EEG Classification & 50-50 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .81,  .87,  1} \textbf{EEG2} & 2     & 64    & 256   & EEG Classification & 20-80 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .81,  .87,  1} \textbf{HT Sensor} & 3     & 11    & 5396  & Food Classification & 50-50 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .81,  .87,  1} \textbf{Movement AAL} & 2     & 4     & 119   & Movement Classification & 50-50 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .81,  .87,  1} \textbf{Occupancy} & 2     & 5     & 3758  & Occupancy Classification & 35-65 split & \cite{Lichman:2013} \\
    \hline
    \rowcolor[rgb]{ .81,  .87,  1} \textbf{Ozone} & 2     & 72    & 291   & Weather Classification & 50-50 split & \cite{Lichman:2013} \\
    \hline

\end{tabularx}
\end{adjustbox}

\end{table*}

==> other_performance_table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
 \newcolumntype{C}{>{\centering\arraybackslash}X}
 \newcommand\mcxl[1]{\multicolumn{1}{|C|}{\bfseries #1}}
 \newcommand\mcx[1]{\multicolumn{1}{C }{\bfseries #1}}
 %\renewcommand*{\thefootnote}{\alph{footnote}}

% \def\tabularxcolumn#1{m{#1}}

%\textbf{*} denotes best model with performance surpassing state-of-the-art results.
%\makesavenoteenv{table*}
 
%\onecolumn
%\begin{supertabular*}{} 
\begin{table*}[]
 \centering
 \caption[Performance comparison of proposed models with the rest on multivariate datasets from various online   database. ]{ Performance comparison of proposed models with the rest on multivariate datasets from various online   database. Green cells denote model with best performance. * denotes best model.
}

\label{tab:perf_tab}
%\begin{minipage*}{\textwidth}
\begin{adjustbox}{width=1 \linewidth}

 \begin{tabularx}{1 \textwidth}{|C|C|C|C|C|C|}
        \hline
         & \textbf{LSTM-FCN} & \textbf{MLSTM-FCN} & \textbf{ALSTM-FCN} & \textbf{MALSTM-FCN} & \textbf{Baseline} \\
    % \hline
    % \textbf{AREM} & 89.74 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{92.31} & 82.05 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{92.31} & 76.92 [DTW]\\
    % \hline
    % \textbf{Daily Sport} & 99.65 & 99.65 & 99.63 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{99.72} & 98.42 [DTW] \\
    % \hline
    % \textbf{EEG} & 60.94 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{65.63} & 64.06 & 64.07 & 62.50 [RF]\\
    % \hline
    % \textbf{EEG2} & 90.67 & 91.00 & 90.67 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{91.33} & 77.50 [RF]\\
    % \hline
    % \textbf{Gesture Phase} & 50.51 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{53.53} & 52.53 & 53.05 & 40.91 [DTW]\\
    % \hline
    % \textbf{HAR} & 96.00 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{96.71} & 95.49 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{96.71} & 81.57 [RF]\\
    % \hline
    % \textbf{HT Sensor} & 68.00 & 78.00 & 72.00 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{80.00} & 72.00 [DTW]\\
    % \hline
    % %\textbf{Japanese Vowels} & 98.65 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{99.19} & 97.84 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{99.19} & 82.16 \\
    % %\hline
    % \textbf{Movement AAL} & 73.25 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{79.63} & 70.06 & 78.34 & 65.61 [SVM-Poly]\\
    % \hline
    % \textbf{Occupancy} & 71.05 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{76.31} & 71.05 & 72.37 & 67.11 [DTW]\\
    % \hline
    % \textbf{Ozone} & 67.63 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{81.50} & 79.19 & 79.78 & 75.14 [DTW]\\
    % %\hline
    % %\textbf{UWave} & 97.65 & 97.91 & 97.88 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{97.93} & 83.58 \\
    % %\hline
    % \hline
    % \textbf{Count} &0.00 & 7.00 & 0.00 & 5.00 & - \\
    % \hline
    
    \hline
    \textbf{AREM} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{89.74} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{92.31*} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{82.05} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{92.31*} & {76.92 [DTW]} \bigstrut\\
    \hline
    \textbf{Daily Sport} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{99.65} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{99.65} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{99.63} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{99.72*} & {98.42 [DTW]} \bigstrut\\
    \hline
    \textbf{EEG} & 60.94 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{65.63*} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{64.06} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{64.07} & {62.50 [RF]} \bigstrut\\
    \hline
    \textbf{EEG2} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{90.67} & \cellcolor[rgb]{ .776,  .878,  .706}{\textbf{91.00}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{90.67} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{91.33*} & {77.50 [RF]} \bigstrut\\
    \hline
    \textbf{Gesture Phase} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{50.51} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{53.53*} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{52.53} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{53.05} & {40.91 [DTW]} \bigstrut\\
    \hline
    \textbf{HAR} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{96.00} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{96.71*} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{95.49} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{96.71*} & {81.57 [RF]} \bigstrut\\
    \hline
    \textbf{HT Sensor} & 68.00 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{78.00} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{72.00} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{80.00*} & {72.00 [DTW]} \bigstrut\\
    \hline
    \textbf{Movement AAL} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{73.25} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{79.63*} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{70.06} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{78.34} & {65.61 [SVM-Poly]} \bigstrut\\
    \hline
    \textbf{Occupancy} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{71.05} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{76.31*} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{71.05} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{72.37} & {67.11 [DTW]} \bigstrut\\
    \hline
    \textbf{Ozone} & 67.63 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{81.50*} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{79.19} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{79.78} & {75.14 [DTW]} \bigstrut\\
    \hline
    \textbf{Count} & 7.00 & 10.00 & 10.00 & 10.00 & - \bigstrut\\
    \hline
    
    \textbf{Arith. Mean} & 3.92  & 1.33  & 3.67  & 1.42  & - \\
    \hline
    \textbf{Geom. Mean} & 3.70  & 1.26  & 3.61  & 1.33  & - \\
    \hline
    \textbf{MPCE} & 8.28  & 6.49  & 7.72  & 6.81  & - \\
    \hline




    %\end{tabularx}%



    \end{tabularx}%
    \end{adjustbox}
    
    %\end{minipage*}
    
  \label{tab:2}%

% \tablefootnote{Green cells designate instances where our performance matches or exceeds state-of-the-art results. \textbf{*} denotes model with best performance.}
%\tablefootnote{Green cells designate instances where our performance matches or exceeds state-of-the-art results. }
%\textbf{*} denotes model with best performance.
%\footnote{Green cells designate instances where our performance matches or exceeds state-of-the-art results.}
\end{table*}%
%\end{supertabular*}
%\twocolumn


==> performance_table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
 \newcolumntype{C}{>{\centering\arraybackslash}X}
 \newcommand\mcxl[1]{\multicolumn{1}{|C|}{\bfseries #1}}
 \newcommand\mcx[1]{\multicolumn{1}{C }{\bfseries #1}}
 \newcolumntype{L}{@{}>{\iffalse}l<{\fi}}


% \def\tabularxcolumn#1{m{#1}}

%\textbf{*} denotes best model with performance surpassing state-of-the-art results.

 \begin{table*}[]
 \centering
 \caption{Performance comparison of proposed models with the rest on benchmark datasets. Green cells denote model with best performance. Red font indicates models that have a strided convolution prior to the LSTM block. * denotes best model.}
\label{tab:perf_tab}
\begin{adjustbox}{width=1 \linewidth}

 \begin{tabularx}{1 \textwidth}{|C|C|C|C|C|C|}
        \hline
          & \textbf{LSTM-FCN} & \textbf{MLSTM-FCN} & \textbf{ALSTM-FCN} & \textbf{MALSTM-FCN} & \textbf{SOTA} \\

    % \hline
    % \textbf{Activity} & 53.13 & 61.88 & 55.63 & \textcolor[rgb]{ 1,  0,  0}{58.75} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{66.25} [DTW] \bigstrut\\
    % \hline
    % \textbf{Action 3d} & 71.72 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{75.42*} & 72.73 & \cellcolor[rgb]{.776,  .878,  .706}\textcolor[rgb]{ 1,  0,  0}{74.74} & 70.71 [DTW] \bigstrut\\
    % \hline
    % \textbf{CK+} &  \cellcolor[rgb]{ .776,  .878,  .706}96.07 &  \cellcolor[rgb]{ .776,  .878,  .706}96.43 &  \cellcolor[rgb]{ .776,  .878,  .706}97.10 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{97.50*} & 93.56 \cite{pei2017multivariate} \bigstrut\\
    % \hline
    % \textbf{Arabic-Voice} &  \cellcolor[rgb]{ .776,  .878,  .706}98.00 &  \cellcolor[rgb]{ .776,  .878,  .706}98.00 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{98.55*} &  \cellcolor[rgb]{ .776,  .878,  .706}98.27 & 94.55  \cite{pei2017multivariate} \bigstrut\\
    % \hline
    % %\textbf{Arabic-Digit} & 99.41 & 99.55 & 99.41 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{99.82} & 96.32 \bigstrut\\
    % %\hline
    % \textbf{OHC} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{99.96*} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{99.96*} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{99.96*} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{99.96*} & 99.03 \cite{jaakkola2000discriminative} \bigstrut\\
    % \hline
    % \textbf{Count} &3.00 & 4.00 & 3.00 & 4.00 & - \\
    % \hline
    % \textbf{Arith. Mean} & 3.20  & 2.00  & 2.00  & 1.40  & - \bigstrut\\
    % \hline
    % \textbf{Geom. Mean} & 2.74  & 2.05  & 1.64  & 1.23  & - \bigstrut\\
    % \hline
    % \textbf{MPCE}  & 0.83  & 0.70  & 0.77  & 0.71  & - \bigstrut\\
    % \hline


    \hline
    {\textbf{Activity}} & 53.13 & 61.88 & 55.63 & \textcolor[rgb]{ 1,  0,  0}{58.75} & {66.25 [DTW]} \bigstrut\\
    \hline
    {\textbf{Action 3d}} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{71.72} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{75.42\textbf{*}} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{72.73} & \cellcolor[rgb]{  .776,  .878,  .706}\textcolor[rgb]{ 1,  0,  0}{\textbf{74.74}} & {70.71 [DTW]} \bigstrut\\
    \hline
    {\textbf{CK+}} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{96.07} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{96.43} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{97.10} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{97.50\textbf{*}} & {93.56 \cite{pei2017multivariate}} \bigstrut\\
    \hline
    {\textbf{Arabic-Voice}} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{98.00} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{98.00} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{98.55\textbf{*}} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{98.27} & {94.55 \cite{pei2017multivariate}} \bigstrut\\
    %\hline
    %{\textbf{Arabic-Digit}} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{99.41} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{99.55} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{99.41} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{99.82} & 96.32 \bigstrut\\
    \hline
    {\textbf{OHC}} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{99.96\textbf{*}} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{99.96\textbf{*}} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{99.96\textbf{*}} & \cellcolor[rgb]{  .776,  .878,  .706}\textbf{99.96\textbf{*}} & {99.03 \cite{pei2017multivariate}} \bigstrut\\
    \hline
    {\textbf{Count}} & 4.00 & 4.00 & 4.00 & 4.00 &  \bigstrut\\
    \hline
    \textbf{Arith. Mean} & 3.20 & 2.00 & 2.00 & 1.40 & - \bigstrut\\
    \hline
    \textbf{Geom. Mean} & 2.74 & 2.05 & 1.64 & 1.23 & - \bigstrut\\
    \hline
    \textbf{MPCE} & 0.83 & 0.70 & 0.77 & 0.71 & - \bigstrut\\
    \hline




    \end{tabularx}
    \end{adjustbox}
  \label{tab:1}%

% \tablefootnote{Green cells designate instances where our performance matches or exceeds state-of-the-art results. \textbf{*} denotes model with best performance.}
\end{table*}%

==> summary_table.tex <==




%\newcolumntype{C}{>{\centering\arraybackslash}X}
% \newcommand\mcxl[1]{\multicolumn{1}{|C|}{\bfseries #1}}
% \newcommand\mcx[1]{\multicolumn{1}{C }{\bfseries #1}}

\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;} 

% \def\tabularxcolumn#1{m{#1}}

 \begin{table}[]
 \centering
 \caption{Summary of advantages of the proposed models}
\label{tab:sum}
\begin{adjustbox}{width=1 \linewidth}

 \begin{tabularx}{0.62 \textwidth}{|C|C|C|C|C|}
    \hline
    Advantage & LSTM-FCN & Refined LSTM-FCN & ALSTM-FCN & Refined ALSTM-FCN \\
    \hline
    Performance &       & \checkmark     &       & \checkmark \\
    \hline
    Visualization &       &       & \checkmark     & \checkmark \\
    \hline
    %\# of Iterations  &       &       & \checkmark     &  \\
    %\hline
    \end{tabularx}
  \end{adjustbox}
\end{table}

==> weasel_dataset.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'


% \def\tabularxcolumn#1{m{#1}}

%\textbf{*} denotes best model with performance surpassing state-of-the-art results.

 \begin{table*}[]
 \centering
 \caption{Performance comparison of proposed models with the rest on 20 benchmark datasets. Green cells denote model with best performance. * denotes best model.}
\label{tab:weasel_tab}
\begin{adjustbox}{width=1 \linewidth}

 \begin{tabularx}{1 \textwidth}{|C|C|C|C|C|C|}

    \hline
    \textbf{Datasets} & \textbf{LSTM-FCN} & \textbf{MLSTM-FCN} & \textbf{ALSTM-FCN} & \textbf{MALSTM-FCN} & \textbf{SOTA} \bigstrut\\
    %\hline
    % \textbf{ArabicDigits} & 1.00  & \cellcolor[rgb]{  .776,  .878,  .706}1.00* & 0.99  & 0.99  & 0.99 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{AUSLAN} & 0.97  & 0.97  & 0.96  & 0.96  & \cellcolor[rgb]{  .776,  .878,  .706}0.98 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{CharacterTrajectories} & 0.99  & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & 0.99  & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & 0.99 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{CMUsubject16} & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 \cite{mvARF} \bigstrut\\
    % \hline
    % \textbf{DigitShapes} & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 \cite{mvARF} \bigstrut\\
    % \hline
    % \textbf{ECG} & 0.85  & 0.86  & 0.86  & 0.86  & \cellcolor[rgb]{  .776,  .878,  .706}0.93 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{JapaneseVowels} & 0.99  & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & 0.99  & 0.99  & 0.98 \cite{ARkernel} \bigstrut\\
    % \hline
    % \textbf{KickvsPunch} & 0.90  & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & 0.90  & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{Libras} & \cellcolor[rgb]{  .776,  .878,  .706}0.99 & 0.97  & 0.98  & 0.97  & 0.95 \cite{ARkernel} \bigstrut\\
    % \hline
    % \textbf{LP1} & 0.74  & 0.86  & 0.80  & 0.82  & \cellcolor[rgb]{  .776,  .878,  .706}0.96 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{LP2} & 0.77  & \cellcolor[rgb]{  .776,  .878,  .706}0.83 & 0.80  & 0.77  & 0.76 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{LP3} & 0.67  & \cellcolor[rgb]{  .776,  .878,  .706}0.80 & \cellcolor[rgb]{  .776,  .878,  .706}0.80 & 0.73  & 0.79 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{LP4} & 0.91  & 0.92  & 0.89  & 0.93  & \cellcolor[rgb]{  .776,  .878,  .706}0.96 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{LP5} & 0.61  & 0.66  & 0.62  & 0.67  & \cellcolor[rgb]{  .776,  .878,  .706}0.71 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{NetFlow} & 0.94  & 0.95  & 0.93  & 0.95  & \cellcolor[rgb]{  .776,  .878,  .706}0.98 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{PenDIgits} & \cellcolor[rgb]{  .776,  .878,  .706}0.97  & \cellcolor[rgb]{  .776,  .878,  .706}0.97  & \cellcolor[rgb]{  .776,  .878,  .706}0.97 & \cellcolor[rgb]{  .776,  .878,  .706}0.97  & 0.95 \cite{ARkernel} \bigstrut\\
    % \hline
    % \textbf{Shapes} & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{UWave} & 0.97  & \cellcolor[rgb]{  .776,  .878,  .706}0.98 & 0.97  & \cellcolor[rgb]{  .776,  .878,  .706}0.98 & \cellcolor[rgb]{  .776,  .878,  .706}0.98 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{Wafer} & \cellcolor[rgb]{  .776,  .878,  .706}0.99 & \cellcolor[rgb]{  .776,  .878,  .706}0.99 & \cellcolor[rgb]{  .776,  .878,  .706}0.99 & \cellcolor[rgb]{  .776,  .878,  .706}0.99 & 0.99 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{WalkvsRun} & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 & \cellcolor[rgb]{  .776,  .878,  .706}1.00 \cite{schafer2017multivariate} \bigstrut\\
    % \hline
    % \textbf{Count} &7.00 & 13.00 & 7.00 & 9.00 & - \\
    % \hline
    
    \hline
    \textbf{ArabicDigits} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.99} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.99} & 0.99 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{AUSLAN} & 0.97 & 0.97 & 0.96 & 0.96 & 0.98 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{CharacterTrajectories} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.99} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.99} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & 0.99 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{CMUsubject16} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & 1.00 \cite{mvARF} \bigstrut\\
    \hline
    \textbf{DigitShapes} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & 1.00 \cite{mvARF} \bigstrut\\
    \hline
    \textbf{ECG} & 0.85 & 0.86 & 0.86 & 0.86 & 0.93 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{JapaneseVowels} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.99} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.99} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.99} & 0.98 \cite{ARkernel} \bigstrut\\
    \hline
    \textbf{KickvsPunch} & 0.90 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & 0.90 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & 1.00 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{Libras} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.99\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.97} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.98} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.97} & 0.95 \cite{ARkernel} \bigstrut\\
    \hline
    \textbf{LP1} & 0.74 & 0.86 & 0.80 & 0.82 & 0.96 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{LP2} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.77} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.83\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.80} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.77} & 0.76 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{LP3} & 0.67 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.80\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.80\textbf{*}} & 0.73 & 0.79 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{LP4} & 0.91 & 0.92 & 0.89 & 0.93 & 0.96 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{LP5} & 0.61 & 0.66 & 0.62 & 0.67 & 0.71 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{NetFlow} & 0.94 & 0.95 & 0.93 & 0.95 & 0.98 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{PenDIgits} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.97\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.97\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.97\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.97\textbf{*}} & 0.95 \cite{ARkernel} \bigstrut\\
    \hline
    \textbf{Shapes} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & 1.00 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{UWave} & 0.97 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.98\textbf{*}} & 0.97 & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.98\textbf{*}} & 0.98 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{Wafer} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.99\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.99\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.99\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{0.99\textbf{*}} & 0.99 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{WalkvsRun} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & \cellcolor[rgb]{ .776,  .878,  .706}\textbf{1.00\textbf{*}} & 1.00 \cite{schafer2017multivariate} \bigstrut\\
    \hline
    \textbf{Count} & 11.00 & 14.00 & 12.00 & 13.00 & - \\
    \hline

    
    \textbf{Arith. Mean} & 4.05  & 2.25  & 3.85  & 3.15  & - \bigstrut\\
    \hline
    \textbf{Geom. Mean} & 2.88  & 1.79  & 2.68  & 2.47  & - \bigstrut\\
    \hline
    \textbf{MPCE} & 0.023  & 0.016  & 0.021  & 0.018  & - \bigstrut\\
    \hline


    \end{tabularx}%
    \end{adjustbox}
  \label{tab:1}%

% \tablefootnote{Green cells designate instances where our performance matches or exceeds state-of-the-art results. \textbf{*} denotes model with best performance.}
\end{table*}%
